Diffusivity of a walk on fractures of a hypertorus

This article studies discrete height functions on the discrete hypertorus. These are functions on the vertices of this hypertorus graph for which the derivative satisfies a specific condition on each edge. We then perform a random walk on the set of such height functions, in the spirit of Diffusivity of a random walk on random walks, a work of Boissard, Cohen, Espinasse, and Norris. The goal is to estimate the diffusivity of this random walk in the mesh limit. It turns out that each height functions is characterised by a number of so-called fractures of the hypertorus. These fractures are then studied in isolation; we are able to understand their asymptotic behaviour in the mesh limit due to the recent understanding of the associated random surfaces. This allows for an asymptotic reduction to a one-dimensional continuous system consisting of $\operatorname{gcd}\mathbf n$ parts where $\mathbf n\in\mathbb N^d$ is the fundamental parameter of the original model. We then prove that the diffusivity of the random walk tends to $1/(1+2\operatorname{gcd}\mathbf n)$ in this mesh limit.

==> figures/large_example_data.tex <==
% !TEX root = ../ms.tex
\qq{40}{40}{4}{50}
\qq{40}{39}{4}{52}
\qq{40}{38}{4}{54}
\qq{40}{37}{4}{56}
\qq{40}{36}{4}{58}
\qq{40}{35}{4}{60}
\qq{40}{34}{4}{62}
\qq{40}{33}{4}{64}
\qq{40}{32}{3}{26}
\qq{40}{31}{3}{28}
\qq{40}{30}{3}{30}
\qq{40}{29}{3}{32}
\qq{40}{28}{3}{34}
\qq{40}{27}{3}{36}
\qq{40}{26}{3}{38}
\qq{40}{25}{3}{40}
\qq{40}{24}{3}{42}
\qq{40}{23}{3}{44}
\qq{40}{22}{3}{46}
\qq{40}{21}{3}{48}
\qq{40}{20}{3}{50}
\qq{40}{19}{3}{52}
\qq{40}{18}{3}{54}
\qq{40}{17}{3}{56}
\qq{40}{16}{3}{58}
\qq{40}{15}{3}{60}
\qq{40}{14}{3}{62}
\qq{40}{13}{3}{64}
\qq{40}{12}{3}{66}
\qq{40}{11}{3}{68}
\qq{40}{10}{3}{70}
\qq{40}{9}{2}{32}
\qq{40}{8}{2}{34}
\qq{40}{7}{2}{36}
\qq{40}{6}{2}{38}
\qq{40}{5}{2}{40}
\qq{40}{4}{2}{42}
\qq{40}{3}{2}{44}
\qq{40}{2}{2}{46}
\qq{40}{1}{2}{48}
\qq{39}{40}{4}{52}
\qq{39}{39}{4}{54}
\qq{39}{38}{4}{56}
\qq{39}{37}{4}{58}
\qq{39}{36}{4}{60}
\qq{39}{35}{4}{62}
\qq{39}{34}{4}{64}
\qq{39}{33}{4}{66}
\qq{39}{32}{3}{28}
\qq{39}{31}{3}{30}
\qq{39}{30}{3}{32}
\qq{39}{29}{3}{34}
\qq{39}{28}{3}{36}
\qq{39}{27}{3}{38}
\qq{39}{26}{3}{40}
\qq{39}{25}{3}{42}
\qq{39}{24}{3}{44}
\qq{39}{23}{3}{46}
\qq{39}{22}{3}{48}
\qq{39}{21}{3}{50}
\qq{39}{20}{3}{52}
\qq{39}{19}{3}{54}
\qq{39}{18}{3}{56}
\qq{39}{17}{3}{58}
\qq{39}{16}{3}{60}
\qq{39}{15}{3}{62}
\qq{39}{14}{3}{64}
\qq{39}{13}{3}{66}
\qq{39}{12}{3}{68}
\qq{39}{11}{3}{70}
\qq{39}{10}{3}{72}
\qq{39}{9}{2}{34}
\qq{39}{8}{2}{36}
\qq{39}{7}{2}{38}
\qq{39}{6}{2}{40}
\qq{39}{5}{2}{42}
\qq{39}{4}{2}{44}
\qq{39}{3}{2}{46}
\qq{39}{2}{2}{48}
\qq{39}{1}{2}{50}
\qq{38}{40}{4}{54}
\qq{38}{39}{4}{56}
\qq{38}{38}{4}{58}
\qq{38}{37}{4}{60}
\qq{38}{36}{4}{62}
\qq{38}{35}{4}{64}
\qq{38}{34}{4}{66}
\qq{38}{33}{4}{68}
\qq{38}{32}{3}{30}
\qq{38}{31}{3}{32}
\qq{38}{30}{3}{34}
\qq{38}{29}{3}{36}
\qq{38}{28}{3}{38}
\qq{38}{27}{3}{40}
\qq{38}{26}{3}{42}
\qq{38}{25}{3}{44}
\qq{38}{24}{3}{46}
\qq{38}{23}{3}{48}
\qq{38}{22}{3}{50}
\qq{38}{21}{3}{52}
\qq{38}{20}{3}{54}
\qq{38}{19}{3}{56}
\qq{38}{18}{3}{58}
\qq{38}{17}{3}{60}
\qq{38}{16}{3}{62}
\qq{38}{15}{3}{64}
\qq{38}{14}{3}{66}
\qq{38}{13}{3}{68}
\qq{38}{12}{3}{70}
\qq{38}{11}{3}{72}
\qq{38}{10}{3}{74}
\qq{38}{9}{2}{36}
\qq{38}{8}{2}{38}
\qq{38}{7}{2}{40}
\qq{38}{6}{2}{42}
\qq{38}{5}{2}{44}
\qq{38}{4}{2}{46}
\qq{38}{3}{2}{48}
\qq{38}{2}{2}{50}
\qq{38}{1}{2}{52}
\qq{37}{40}{4}{56}
\qq{37}{39}{4}{58}
\qq{37}{38}{4}{60}
\qq{37}{37}{4}{62}
\qq{37}{36}{4}{64}
\qq{37}{35}{4}{66}
\qq{37}{34}{4}{68}
\qq{37}{33}{4}{70}
\qq{37}{32}{3}{32}
\qq{37}{31}{3}{34}
\qq{37}{30}{3}{36}
\qq{37}{29}{3}{38}
\qq{37}{28}{3}{40}
\qq{37}{27}{3}{42}
\qq{37}{26}{3}{44}
\qq{37}{25}{3}{46}
\qq{37}{24}{3}{48}
\qq{37}{23}{3}{50}
\qq{37}{22}{3}{52}
\qq{37}{21}{3}{54}
\qq{37}{20}{3}{56}
\qq{37}{19}{3}{58}
\qq{37}{18}{3}{60}
\qq{37}{17}{3}{62}
\qq{37}{16}{3}{64}
\qq{37}{15}{3}{66}
\qq{37}{14}{3}{68}
\qq{37}{13}{3}{70}
\qq{37}{12}{3}{72}
\qq{37}{11}{3}{74}
\qq{37}{10}{2}{36}
\qq{37}{9}{2}{38}
\qq{37}{8}{2}{40}
\qq{37}{7}{2}{42}
\qq{37}{6}{2}{44}
\qq{37}{5}{2}{46}
\qq{37}{4}{2}{48}
\qq{37}{3}{2}{50}
\qq{37}{2}{2}{52}
\qq{37}{1}{2}{54}
\qq{36}{40}{4}{58}
\qq{36}{39}{4}{60}
\qq{36}{38}{4}{62}
\qq{36}{37}{4}{64}
\qq{36}{36}{4}{66}
\qq{36}{35}{4}{68}
\qq{36}{34}{4}{70}
\qq{36}{33}{4}{72}
\qq{36}{32}{3}{34}
\qq{36}{31}{3}{36}
\qq{36}{30}{3}{38}
\qq{36}{29}{3}{40}
\qq{36}{28}{3}{42}
\qq{36}{27}{3}{44}
\qq{36}{26}{3}{46}
\qq{36}{25}{3}{48}
\qq{36}{24}{3}{50}
\qq{36}{23}{3}{52}
\qq{36}{22}{3}{54}
\qq{36}{21}{3}{56}
\qq{36}{20}{3}{58}
\qq{36}{19}{3}{60}
\qq{36}{18}{3}{62}
\qq{36}{17}{3}{64}
\qq{36}{16}{3}{66}
\qq{36}{15}{3}{68}
\qq{36}{14}{2}{30}
\qq{36}{13}{2}{32}
\qq{36}{12}{2}{34}
\qq{36}{11}{2}{36}
\qq{36}{10}{2}{38}
\qq{36}{9}{2}{40}
\qq{36}{8}{2}{42}
\qq{36}{7}{2}{44}
\qq{36}{6}{2}{46}
\qq{36}{5}{2}{48}
\qq{36}{4}{2}{50}
\qq{36}{3}{2}{52}
\qq{36}{2}{2}{54}
\qq{36}{1}{2}{56}
\qq{35}{40}{4}{60}
\qq{35}{39}{4}{62}
\qq{35}{38}{4}{64}
\qq{35}{37}{4}{66}
\qq{35}{36}{4}{68}
\qq{35}{35}{4}{70}
\qq{35}{34}{4}{72}
\qq{35}{33}{3}{34}
\qq{35}{32}{3}{36}
\qq{35}{31}{3}{38}
\qq{35}{30}{3}{40}
\qq{35}{29}{3}{42}
\qq{35}{28}{3}{44}
\qq{35}{27}{3}{46}
\qq{35}{26}{3}{48}
\qq{35}{25}{3}{50}
\qq{35}{24}{3}{52}
\qq{35}{23}{3}{54}
\qq{35}{22}{3}{56}
\qq{35}{21}{3}{58}
\qq{35}{20}{3}{60}
\qq{35}{19}{3}{62}
\qq{35}{18}{3}{64}
\qq{35}{17}{3}{66}
\qq{35}{16}{3}{68}
\qq{35}{15}{3}{70}
\qq{35}{14}{2}{32}
\qq{35}{13}{2}{34}
\qq{35}{12}{2}{36}
\qq{35}{11}{2}{38}
\qq{35}{10}{2}{40}
\qq{35}{9}{2}{42}
\qq{35}{8}{2}{44}
\qq{35}{7}{2}{46}
\qq{35}{6}{2}{48}
\qq{35}{5}{2}{50}
\qq{35}{4}{2}{52}
\qq{35}{3}{2}{54}
\qq{35}{2}{2}{56}
\qq{35}{1}{2}{58}
\qq{34}{40}{4}{62}
\qq{34}{39}{4}{64}
\qq{34}{38}{4}{66}
\qq{34}{37}{4}{68}
\qq{34}{36}{4}{70}
\qq{34}{35}{4}{72}
\qq{34}{34}{4}{74}
\qq{34}{33}{3}{36}
\qq{34}{32}{3}{38}
\qq{34}{31}{3}{40}
\qq{34}{30}{3}{42}
\qq{34}{29}{3}{44}
\qq{34}{28}{3}{46}
\qq{34}{27}{3}{48}
\qq{34}{26}{3}{50}
\qq{34}{25}{3}{52}
\qq{34}{24}{3}{54}
\qq{34}{23}{3}{56}
\qq{34}{22}{3}{58}
\qq{34}{21}{3}{60}
\qq{34}{20}{3}{62}
\qq{34}{19}{3}{64}
\qq{34}{18}{3}{66}
\qq{34}{17}{3}{68}
\qq{34}{16}{3}{70}
\qq{34}{15}{3}{72}
\qq{34}{14}{2}{34}
\qq{34}{13}{2}{36}
\qq{34}{12}{2}{38}
\qq{34}{11}{2}{40}
\qq{34}{10}{2}{42}
\qq{34}{9}{2}{44}
\qq{34}{8}{2}{46}
\qq{34}{7}{2}{48}
\qq{34}{6}{2}{50}
\qq{34}{5}{2}{52}
\qq{34}{4}{2}{54}
\qq{34}{3}{2}{56}
\qq{34}{2}{2}{58}
\qq{34}{1}{2}{60}
\qq{33}{40}{4}{64}
\qq{33}{39}{4}{66}
\qq{33}{38}{4}{68}
\qq{33}{37}{4}{70}
\qq{33}{36}{4}{72}
\qq{33}{35}{4}{74}
\qq{33}{34}{4}{76}
\qq{33}{33}{3}{38}
\qq{33}{32}{3}{40}
\qq{33}{31}{3}{42}
\qq{33}{30}{3}{44}
\qq{33}{29}{3}{46}
\qq{33}{28}{3}{48}
\qq{33}{27}{3}{50}
\qq{33}{26}{3}{52}
\qq{33}{25}{3}{54}
\qq{33}{24}{3}{56}
\qq{33}{23}{3}{58}
\qq{33}{22}{3}{60}
\qq{33}{21}{3}{62}
\qq{33}{20}{3}{64}
\qq{33}{19}{3}{66}
\qq{33}{18}{3}{68}
\qq{33}{17}{3}{70}
\qq{33}{16}{3}{72}
\qq{33}{15}{2}{34}
\qq{33}{14}{2}{36}
\qq{33}{13}{2}{38}
\qq{33}{12}{2}{40}
\qq{33}{11}{2}{42}
\qq{33}{10}{2}{44}
\qq{33}{9}{2}{46}
\qq{33}{8}{2}{48}
\qq{33}{7}{2}{50}
\qq{33}{6}{2}{52}
\qq{33}{5}{2}{54}
\qq{33}{4}{2}{56}
\qq{33}{3}{2}{58}
\qq{33}{2}{2}{60}
\qq{33}{1}{2}{62}
\qq{32}{40}{4}{66}
\qq{32}{39}{4}{68}
\qq{32}{38}{4}{70}
\qq{32}{37}{4}{72}
\qq{32}{36}{4}{74}
\qq{32}{35}{4}{76}
\qq{32}{34}{3}{38}
\qq{32}{33}{3}{40}
\qq{32}{32}{3}{42}
\qq{32}{31}{3}{44}
\qq{32}{30}{3}{46}
\qq{32}{29}{3}{48}
\qq{32}{28}{3}{50}
\qq{32}{27}{3}{52}
\qq{32}{26}{3}{54}
\qq{32}{25}{3}{56}
\qq{32}{24}{3}{58}
\qq{32}{23}{3}{60}
\qq{32}{22}{3}{62}
\qq{32}{21}{3}{64}
\qq{32}{20}{3}{66}
\qq{32}{19}{3}{68}
\qq{32}{18}{3}{70}
\qq{32}{17}{3}{72}
\qq{32}{16}{2}{34}
\qq{32}{15}{2}{36}
\qq{32}{14}{2}{38}
\qq{32}{13}{2}{40}
\qq{32}{12}{2}{42}
\qq{32}{11}{2}{44}
\qq{32}{10}{2}{46}
\qq{32}{9}{2}{48}
\qq{32}{8}{2}{50}
\qq{32}{7}{2}{52}
\qq{32}{6}{2}{54}
\qq{32}{5}{2}{56}
\qq{32}{4}{2}{58}
\qq{32}{3}{2}{60}
\qq{32}{2}{2}{62}
\qq{32}{1}{2}{64}
\qq{31}{40}{4}{68}
\qq{31}{39}{4}{70}
\qq{31}{38}{4}{72}
\qq{31}{37}{4}{74}
\qq{31}{36}{4}{76}
\qq{31}{35}{4}{78}
\qq{31}{34}{3}{40}
\qq{31}{33}{3}{42}
\qq{31}{32}{3}{44}
\qq{31}{31}{3}{46}
\qq{31}{30}{3}{48}
\qq{31}{29}{3}{50}
\qq{31}{28}{3}{52}
\qq{31}{27}{3}{54}
\qq{31}{26}{3}{56}
\qq{31}{25}{3}{58}
\qq{31}{24}{3}{60}
\qq{31}{23}{3}{62}
\qq{31}{22}{3}{64}
\qq{31}{21}{3}{66}
\qq{31}{20}{3}{68}
\qq{31}{19}{3}{70}
\qq{31}{18}{3}{72}
\qq{31}{17}{2}{34}
\qq{31}{16}{2}{36}
\qq{31}{15}{2}{38}
\qq{31}{14}{2}{40}
\qq{31}{13}{2}{42}
\qq{31}{12}{2}{44}
\qq{31}{11}{2}{46}
\qq{31}{10}{2}{48}
\qq{31}{9}{2}{50}
\qq{31}{8}{2}{52}
\qq{31}{7}{2}{54}
\qq{31}{6}{2}{56}
\qq{31}{5}{2}{58}
\qq{31}{4}{2}{60}
\qq{31}{3}{2}{62}
\qq{31}{2}{2}{64}
\qq{31}{1}{2}{66}
\qq{30}{40}{4}{70}
\qq{30}{39}{4}{72}
\qq{30}{38}{4}{74}
\qq{30}{37}{3}{36}
\qq{30}{36}{3}{38}
\qq{30}{35}{3}{40}
\qq{30}{34}{3}{42}
\qq{30}{33}{3}{44}
\qq{30}{32}{3}{46}
\qq{30}{31}{3}{48}
\qq{30}{30}{3}{50}
\qq{30}{29}{3}{52}
\qq{30}{28}{3}{54}
\qq{30}{27}{3}{56}
\qq{30}{26}{3}{58}
\qq{30}{25}{3}{60}
\qq{30}{24}{3}{62}
\qq{30}{23}{3}{64}
\qq{30}{22}{3}{66}
\qq{30}{21}{3}{68}
\qq{30}{20}{3}{70}
\qq{30}{19}{3}{72}
\qq{30}{18}{3}{74}
\qq{30}{17}{2}{36}
\qq{30}{16}{2}{38}
\qq{30}{15}{2}{40}
\qq{30}{14}{2}{42}
\qq{30}{13}{2}{44}
\qq{30}{12}{2}{46}
\qq{30}{11}{2}{48}
\qq{30}{10}{2}{50}
\qq{30}{9}{2}{52}
\qq{30}{8}{2}{54}
\qq{30}{7}{2}{56}
\qq{30}{6}{2}{58}
\qq{30}{5}{2}{60}
\qq{30}{4}{2}{62}
\qq{30}{3}{2}{64}
\qq{30}{2}{2}{66}
\qq{30}{1}{2}{68}
\qq{29}{40}{4}{72}
\qq{29}{39}{4}{74}
\qq{29}{38}{4}{76}
\qq{29}{37}{3}{38}
\qq{29}{36}{3}{40}
\qq{29}{35}{3}{42}
\qq{29}{34}{3}{44}
\qq{29}{33}{3}{46}
\qq{29}{32}{3}{48}
\qq{29}{31}{3}{50}
\qq{29}{30}{3}{52}
\qq{29}{29}{3}{54}
\qq{29}{28}{3}{56}
\qq{29}{27}{3}{58}
\qq{29}{26}{3}{60}
\qq{29}{25}{3}{62}
\qq{29}{24}{3}{64}
\qq{29}{23}{3}{66}
\qq{29}{22}{3}{68}
\qq{29}{21}{3}{70}
\qq{29}{20}{3}{72}
\qq{29}{19}{3}{74}
\qq{29}{18}{3}{76}
\qq{29}{17}{2}{38}
\qq{29}{16}{2}{40}
\qq{29}{15}{2}{42}
\qq{29}{14}{2}{44}
\qq{29}{13}{2}{46}
\qq{29}{12}{2}{48}
\qq{29}{11}{2}{50}
\qq{29}{10}{2}{52}
\qq{29}{9}{2}{54}
\qq{29}{8}{2}{56}
\qq{29}{7}{2}{58}
\qq{29}{6}{2}{60}
\qq{29}{5}{2}{62}
\qq{29}{4}{2}{64}
\qq{29}{3}{2}{66}
\qq{29}{2}{2}{68}
\qq{29}{1}{2}{70}
\qq{28}{40}{4}{74}
\qq{28}{39}{4}{76}
\qq{28}{38}{4}{78}
\qq{28}{37}{3}{40}
\qq{28}{36}{3}{42}
\qq{28}{35}{3}{44}
\qq{28}{34}{3}{46}
\qq{28}{33}{3}{48}
\qq{28}{32}{3}{50}
\qq{28}{31}{3}{52}
\qq{28}{30}{3}{54}
\qq{28}{29}{3}{56}
\qq{28}{28}{3}{58}
\qq{28}{27}{3}{60}
\qq{28}{26}{3}{62}
\qq{28}{25}{3}{64}
\qq{28}{24}{3}{66}
\qq{28}{23}{3}{68}
\qq{28}{22}{3}{70}
\qq{28}{21}{3}{72}
\qq{28}{20}{3}{74}
\qq{28}{19}{3}{76}
\qq{28}{18}{3}{78}
\qq{28}{17}{2}{40}
\qq{28}{16}{2}{42}
\qq{28}{15}{2}{44}
\qq{28}{14}{2}{46}
\qq{28}{13}{2}{48}
\qq{28}{12}{2}{50}
\qq{28}{11}{2}{52}
\qq{28}{10}{2}{54}
\qq{28}{9}{2}{56}
\qq{28}{8}{2}{58}
\qq{28}{7}{2}{60}
\qq{28}{6}{2}{62}
\qq{28}{5}{2}{64}
\qq{28}{4}{2}{66}
\qq{28}{3}{2}{68}
\qq{28}{2}{2}{70}
\qq{28}{1}{2}{72}
\qq{27}{40}{4}{76}
\qq{27}{39}{4}{78}
\qq{27}{38}{4}{80}
\qq{27}{37}{3}{42}
\qq{27}{36}{3}{44}
\qq{27}{35}{3}{46}
\qq{27}{34}{3}{48}
\qq{27}{33}{3}{50}
\qq{27}{32}{3}{52}
\qq{27}{31}{3}{54}
\qq{27}{30}{3}{56}
\qq{27}{29}{3}{58}
\qq{27}{28}{3}{60}
\qq{27}{27}{3}{62}
\qq{27}{26}{3}{64}
\qq{27}{25}{3}{66}
\qq{27}{24}{3}{68}
\qq{27}{23}{3}{70}
\qq{27}{22}{3}{72}
\qq{27}{21}{3}{74}
\qq{27}{20}{3}{76}
\qq{27}{19}{3}{78}
\qq{27}{18}{2}{40}
\qq{27}{17}{2}{42}
\qq{27}{16}{2}{44}
\qq{27}{15}{2}{46}
\qq{27}{14}{2}{48}
\qq{27}{13}{2}{50}
\qq{27}{12}{2}{52}
\qq{27}{11}{2}{54}
\qq{27}{10}{2}{56}
\qq{27}{9}{2}{58}
\qq{27}{8}{2}{60}
\qq{27}{7}{2}{62}
\qq{27}{6}{2}{64}
\qq{27}{5}{2}{66}
\qq{27}{4}{2}{68}
\qq{27}{3}{2}{70}
\qq{27}{2}{2}{72}
\qq{27}{1}{2}{74}
\qq{26}{40}{4}{78}
\qq{26}{39}{4}{80}
\qq{26}{38}{4}{82}
\qq{26}{37}{3}{44}
\qq{26}{36}{3}{46}
\qq{26}{35}{3}{48}
\qq{26}{34}{3}{50}
\qq{26}{33}{3}{52}
\qq{26}{32}{3}{54}
\qq{26}{31}{3}{56}
\qq{26}{30}{3}{58}
\qq{26}{29}{3}{60}
\qq{26}{28}{3}{62}
\qq{26}{27}{3}{64}
\qq{26}{26}{3}{66}
\qq{26}{25}{3}{68}
\qq{26}{24}{3}{70}
\qq{26}{23}{3}{72}
\qq{26}{22}{3}{74}
\qq{26}{21}{3}{76}
\qq{26}{20}{3}{78}
\qq{26}{19}{3}{80}
\qq{26}{18}{2}{42}
\qq{26}{17}{2}{44}
\qq{26}{16}{2}{46}
\qq{26}{15}{2}{48}
\qq{26}{14}{2}{50}
\qq{26}{13}{2}{52}
\qq{26}{12}{2}{54}
\qq{26}{11}{2}{56}
\qq{26}{10}{2}{58}
\qq{26}{9}{2}{60}
\qq{26}{8}{2}{62}
\qq{26}{7}{2}{64}
\qq{26}{6}{2}{66}
\qq{26}{5}{2}{68}
\qq{26}{4}{2}{70}
\qq{26}{3}{2}{72}
\qq{26}{2}{2}{74}
\qq{26}{1}{2}{76}
\qq{25}{40}{4}{80}
\qq{25}{39}{4}{82}
\qq{25}{38}{4}{84}
\qq{25}{37}{3}{46}
\qq{25}{36}{3}{48}
\qq{25}{35}{3}{50}
\qq{25}{34}{3}{52}
\qq{25}{33}{3}{54}
\qq{25}{32}{3}{56}
\qq{25}{31}{3}{58}
\qq{25}{30}{3}{60}
\qq{25}{29}{3}{62}
\qq{25}{28}{3}{64}
\qq{25}{27}{3}{66}
\qq{25}{26}{3}{68}
\qq{25}{25}{3}{70}
\qq{25}{24}{3}{72}
\qq{25}{23}{3}{74}
\qq{25}{22}{3}{76}
\qq{25}{21}{3}{78}
\qq{25}{20}{2}{40}
\qq{25}{19}{2}{42}
\qq{25}{18}{2}{44}
\qq{25}{17}{2}{46}
\qq{25}{16}{2}{48}
\qq{25}{15}{2}{50}
\qq{25}{14}{2}{52}
\qq{25}{13}{2}{54}
\qq{25}{12}{2}{56}
\qq{25}{11}{2}{58}
\qq{25}{10}{2}{60}
\qq{25}{9}{2}{62}
\qq{25}{8}{2}{64}
\qq{25}{7}{2}{66}
\qq{25}{6}{2}{68}
\qq{25}{5}{2}{70}
\qq{25}{4}{2}{72}
\qq{25}{3}{2}{74}
\qq{25}{2}{2}{76}
\qq{25}{1}{2}{78}
\qq{24}{40}{4}{82}
\qq{24}{39}{4}{84}
\qq{24}{38}{3}{46}
\qq{24}{37}{3}{48}
\qq{24}{36}{3}{50}
\qq{24}{35}{3}{52}
\qq{24}{34}{3}{54}
\qq{24}{33}{3}{56}
\qq{24}{32}{3}{58}
\qq{24}{31}{3}{60}
\qq{24}{30}{3}{62}
\qq{24}{29}{3}{64}
\qq{24}{28}{3}{66}
\qq{24}{27}{3}{68}
\qq{24}{26}{3}{70}
\qq{24}{25}{3}{72}
\qq{24}{24}{3}{74}
\qq{24}{23}{3}{76}
\qq{24}{22}{3}{78}
\qq{24}{21}{3}{80}
\qq{24}{20}{2}{42}
\qq{24}{19}{2}{44}
\qq{24}{18}{2}{46}
\qq{24}{17}{2}{48}
\qq{24}{16}{2}{50}
\qq{24}{15}{2}{52}
\qq{24}{14}{2}{54}
\qq{24}{13}{2}{56}
\qq{24}{12}{2}{58}
\qq{24}{11}{2}{60}
\qq{24}{10}{2}{62}
\qq{24}{9}{2}{64}
\qq{24}{8}{2}{66}
\qq{24}{7}{2}{68}
\qq{24}{6}{2}{70}
\qq{24}{5}{2}{72}
\qq{24}{4}{2}{74}
\qq{24}{3}{2}{76}
\qq{24}{2}{2}{78}
\qq{24}{1}{2}{80}
\qq{23}{40}{4}{84}
\qq{23}{39}{4}{86}
\qq{23}{38}{3}{48}
\qq{23}{37}{3}{50}
\qq{23}{36}{3}{52}
\qq{23}{35}{3}{54}
\qq{23}{34}{3}{56}
\qq{23}{33}{3}{58}
\qq{23}{32}{3}{60}
\qq{23}{31}{3}{62}
\qq{23}{30}{3}{64}
\qq{23}{29}{3}{66}
\qq{23}{28}{3}{68}
\qq{23}{27}{3}{70}
\qq{23}{26}{3}{72}
\qq{23}{25}{3}{74}
\qq{23}{24}{3}{76}
\qq{23}{23}{3}{78}
\qq{23}{22}{3}{80}
\qq{23}{21}{2}{42}
\qq{23}{20}{2}{44}
\qq{23}{19}{2}{46}
\qq{23}{18}{2}{48}
\qq{23}{17}{2}{50}
\qq{23}{16}{2}{52}
\qq{23}{15}{2}{54}
\qq{23}{14}{2}{56}
\qq{23}{13}{2}{58}
\qq{23}{12}{2}{60}
\qq{23}{11}{2}{62}
\qq{23}{10}{2}{64}
\qq{23}{9}{2}{66}
\qq{23}{8}{2}{68}
\qq{23}{7}{2}{70}
\qq{23}{6}{2}{72}
\qq{23}{5}{2}{74}
\qq{23}{4}{2}{76}
\qq{23}{3}{2}{78}
\qq{23}{2}{2}{80}
\qq{23}{1}{2}{82}
\qq{22}{40}{4}{86}
\qq{22}{39}{4}{88}
\qq{22}{38}{3}{50}
\qq{22}{37}{3}{52}
\qq{22}{36}{3}{54}
\qq{22}{35}{3}{56}
\qq{22}{34}{3}{58}
\qq{22}{33}{3}{60}
\qq{22}{32}{3}{62}
\qq{22}{31}{3}{64}
\qq{22}{30}{3}{66}
\qq{22}{29}{3}{68}
\qq{22}{28}{3}{70}
\qq{22}{27}{3}{72}
\qq{22}{26}{3}{74}
\qq{22}{25}{3}{76}
\qq{22}{24}{3}{78}
\qq{22}{23}{2}{40}
\qq{22}{22}{2}{42}
\qq{22}{21}{2}{44}
\qq{22}{20}{2}{46}
\qq{22}{19}{2}{48}
\qq{22}{18}{2}{50}
\qq{22}{17}{2}{52}
\qq{22}{16}{2}{54}
\qq{22}{15}{2}{56}
\qq{22}{14}{2}{58}
\qq{22}{13}{2}{60}
\qq{22}{12}{2}{62}
\qq{22}{11}{2}{64}
\qq{22}{10}{2}{66}
\qq{22}{9}{2}{68}
\qq{22}{8}{2}{70}
\qq{22}{7}{2}{72}
\qq{22}{6}{2}{74}
\qq{22}{5}{2}{76}
\qq{22}{4}{2}{78}
\qq{22}{3}{2}{80}
\qq{22}{2}{2}{82}
\qq{22}{1}{2}{84}
\qq{21}{40}{4}{88}
\qq{21}{39}{4}{90}
\qq{21}{38}{3}{52}
\qq{21}{37}{3}{54}
\qq{21}{36}{3}{56}
\qq{21}{35}{3}{58}
\qq{21}{34}{3}{60}
\qq{21}{33}{3}{62}
\qq{21}{32}{3}{64}
\qq{21}{31}{3}{66}
\qq{21}{30}{3}{68}
\qq{21}{29}{3}{70}
\qq{21}{28}{3}{72}
\qq{21}{27}{3}{74}
\qq{21}{26}{3}{76}
\qq{21}{25}{2}{38}
\qq{21}{24}{2}{40}
\qq{21}{23}{2}{42}
\qq{21}{22}{2}{44}
\qq{21}{21}{2}{46}
\qq{21}{20}{2}{48}
\qq{21}{19}{2}{50}
\qq{21}{18}{2}{52}
\qq{21}{17}{2}{54}
\qq{21}{16}{2}{56}
\qq{21}{15}{2}{58}
\qq{21}{14}{2}{60}
\qq{21}{13}{2}{62}
\qq{21}{12}{2}{64}
\qq{21}{11}{2}{66}
\qq{21}{10}{2}{68}
\qq{21}{9}{2}{70}
\qq{21}{8}{2}{72}
\qq{21}{7}{2}{74}
\qq{21}{6}{2}{76}
\qq{21}{5}{2}{78}
\qq{21}{4}{2}{80}
\qq{21}{3}{2}{82}
\qq{21}{2}{2}{84}
\qq{21}{1}{2}{86}
\qq{21}{40}{4}{88}
\qq{21}{39}{4}{90}
\qq{21}{38}{3}{52}
\qq{21}{37}{3}{54}
\qq{21}{36}{3}{56}
\qq{21}{35}{3}{58}
\qq{21}{34}{3}{60}
\qq{21}{33}{3}{62}
\qq{21}{32}{3}{64}
\qq{21}{31}{3}{66}
\qq{21}{30}{3}{68}
\qq{21}{29}{3}{70}
\qq{21}{28}{3}{72}
\qq{21}{27}{3}{74}
\qq{21}{26}{3}{76}
\qq{21}{25}{2}{38}
\qq{21}{24}{2}{40}
\qq{21}{23}{2}{42}
\qq{21}{22}{2}{44}
\qq{21}{21}{2}{46}
\qq{21}{20}{2}{48}
\qq{21}{19}{2}{50}
\qq{21}{18}{2}{52}
\qq{21}{17}{2}{54}
\qq{21}{16}{2}{56}
\qq{21}{15}{2}{58}
\qq{21}{14}{2}{60}
\qq{21}{13}{2}{62}
\qq{21}{12}{2}{64}
\qq{21}{11}{2}{66}
\qq{21}{10}{2}{68}
\qq{21}{9}{2}{70}
\qq{21}{8}{2}{72}
\qq{21}{7}{2}{74}
\qq{21}{6}{2}{76}
\qq{21}{5}{2}{78}
\qq{21}{4}{2}{80}
\qq{21}{3}{2}{82}
\qq{21}{2}{2}{84}
\qq{21}{1}{2}{86}
\qq{20}{40}{4}{90}
\qq{20}{39}{3}{52}
\qq{20}{38}{3}{54}
\qq{20}{37}{3}{56}
\qq{20}{36}{3}{58}
\qq{20}{35}{3}{60}
\qq{20}{34}{3}{62}
\qq{20}{33}{3}{64}
\qq{20}{32}{3}{66}
\qq{20}{31}{3}{68}
\qq{20}{30}{3}{70}
\qq{20}{29}{3}{72}
\qq{20}{28}{3}{74}
\qq{20}{27}{3}{76}
\qq{20}{26}{3}{78}
\qq{20}{25}{2}{40}
\qq{20}{24}{2}{42}
\qq{20}{23}{2}{44}
\qq{20}{22}{2}{46}
\qq{20}{21}{2}{48}
\qq{20}{20}{2}{50}
\qq{20}{19}{2}{52}
\qq{20}{18}{2}{54}
\qq{20}{17}{2}{56}
\qq{20}{16}{2}{58}
\qq{20}{15}{2}{60}
\qq{20}{14}{2}{62}
\qq{20}{13}{2}{64}
\qq{20}{12}{2}{66}
\qq{20}{11}{2}{68}
\qq{20}{10}{2}{70}
\qq{20}{9}{2}{72}
\qq{20}{8}{2}{74}
\qq{20}{7}{2}{76}
\qq{20}{6}{2}{78}
\qq{20}{5}{2}{80}
\qq{20}{4}{2}{82}
\qq{20}{3}{2}{84}
\qq{20}{2}{2}{86}
\qq{20}{1}{2}{88}
\qq{19}{40}{3}{52}
\qq{19}{39}{3}{54}
\qq{19}{38}{3}{56}
\qq{19}{37}{3}{58}
\qq{19}{36}{3}{60}
\qq{19}{35}{3}{62}
\qq{19}{34}{3}{64}
\qq{19}{33}{3}{66}
\qq{19}{32}{3}{68}
\qq{19}{31}{3}{70}
\qq{19}{30}{3}{72}
\qq{19}{29}{3}{74}
\qq{19}{28}{3}{76}
\qq{19}{27}{3}{78}
\qq{19}{26}{3}{80}
\qq{19}{25}{2}{42}
\qq{19}{24}{2}{44}
\qq{19}{23}{2}{46}
\qq{19}{22}{2}{48}
\qq{19}{21}{2}{50}
\qq{19}{20}{2}{52}
\qq{19}{19}{2}{54}
\qq{19}{18}{2}{56}
\qq{19}{17}{2}{58}
\qq{19}{16}{2}{60}
\qq{19}{15}{2}{62}
\qq{19}{14}{2}{64}
\qq{19}{13}{2}{66}
\qq{19}{12}{2}{68}
\qq{19}{11}{2}{70}
\qq{19}{10}{2}{72}
\qq{19}{9}{2}{74}
\qq{19}{8}{2}{76}
\qq{19}{7}{2}{78}
\qq{19}{6}{2}{80}
\qq{19}{5}{2}{82}
\qq{19}{4}{2}{84}
\qq{19}{3}{2}{86}
\qq{19}{2}{1}{48}
\qq{19}{1}{1}{50}
\qq{18}{40}{3}{54}
\qq{18}{39}{3}{56}
\qq{18}{38}{3}{58}
\qq{18}{37}{3}{60}
\qq{18}{36}{3}{62}
\qq{18}{35}{3}{64}
\qq{18}{34}{3}{66}
\qq{18}{33}{3}{68}
\qq{18}{32}{3}{70}
\qq{18}{31}{3}{72}
\qq{18}{30}{3}{74}
\qq{18}{29}{3}{76}
\qq{18}{28}{3}{78}
\qq{18}{27}{3}{80}
\qq{18}{26}{3}{82}
\qq{18}{25}{2}{44}
\qq{18}{24}{2}{46}
\qq{18}{23}{2}{48}
\qq{18}{22}{2}{50}
\qq{18}{21}{2}{52}
\qq{18}{20}{2}{54}
\qq{18}{19}{2}{56}
\qq{18}{18}{2}{58}
\qq{18}{17}{2}{60}
\qq{18}{16}{2}{62}
\qq{18}{15}{2}{64}
\qq{18}{14}{2}{66}
\qq{18}{13}{2}{68}
\qq{18}{12}{2}{70}
\qq{18}{11}{2}{72}
\qq{18}{10}{2}{74}
\qq{18}{9}{2}{76}
\qq{18}{8}{2}{78}
\qq{18}{7}{2}{80}
\qq{18}{6}{2}{82}
\qq{18}{5}{1}{44}
\qq{18}{4}{1}{46}
\qq{18}{3}{1}{48}
\qq{18}{2}{1}{50}
\qq{18}{1}{1}{52}
\qq{17}{40}{3}{56}
\qq{17}{39}{3}{58}
\qq{17}{38}{3}{60}
\qq{17}{37}{3}{62}
\qq{17}{36}{3}{64}
\qq{17}{35}{3}{66}
\qq{17}{34}{3}{68}
\qq{17}{33}{3}{70}
\qq{17}{32}{3}{72}
\qq{17}{31}{3}{74}
\qq{17}{30}{3}{76}
\qq{17}{29}{3}{78}
\qq{17}{28}{3}{80}
\qq{17}{27}{2}{42}
\qq{17}{26}{2}{44}
\qq{17}{25}{2}{46}
\qq{17}{24}{2}{48}
\qq{17}{23}{2}{50}
\qq{17}{22}{2}{52}
\qq{17}{21}{2}{54}
\qq{17}{20}{2}{56}
\qq{17}{19}{2}{58}
\qq{17}{18}{2}{60}
\qq{17}{17}{2}{62}
\qq{17}{16}{2}{64}
\qq{17}{15}{2}{66}
\qq{17}{14}{2}{68}
\qq{17}{13}{2}{70}
\qq{17}{12}{2}{72}
\qq{17}{11}{2}{74}
\qq{17}{10}{2}{76}
\qq{17}{9}{2}{78}
\qq{17}{8}{2}{80}
\qq{17}{7}{1}{42}
\qq{17}{6}{1}{44}
\qq{17}{5}{1}{46}
\qq{17}{4}{1}{48}
\qq{17}{3}{1}{50}
\qq{17}{2}{1}{52}
\qq{17}{1}{1}{54}
\qq{16}{40}{3}{58}
\qq{16}{39}{3}{60}
\qq{16}{38}{3}{62}
\qq{16}{37}{3}{64}
\qq{16}{36}{3}{66}
\qq{16}{35}{3}{68}
\qq{16}{34}{3}{70}
\qq{16}{33}{3}{72}
\qq{16}{32}{3}{74}
\qq{16}{31}{3}{76}
\qq{16}{30}{3}{78}
\qq{16}{29}{2}{40}
\qq{16}{28}{2}{42}
\qq{16}{27}{2}{44}
\qq{16}{26}{2}{46}
\qq{16}{25}{2}{48}
\qq{16}{24}{2}{50}
\qq{16}{23}{2}{52}
\qq{16}{22}{2}{54}
\qq{16}{21}{2}{56}
\qq{16}{20}{2}{58}
\qq{16}{19}{2}{60}
\qq{16}{18}{2}{62}
\qq{16}{17}{2}{64}
\qq{16}{16}{2}{66}
\qq{16}{15}{2}{68}
\qq{16}{14}{2}{70}
\qq{16}{13}{2}{72}
\qq{16}{12}{2}{74}
\qq{16}{11}{2}{76}
\qq{16}{10}{2}{78}
\qq{16}{9}{2}{80}
\qq{16}{8}{1}{42}
\qq{16}{7}{1}{44}
\qq{16}{6}{1}{46}
\qq{16}{5}{1}{48}
\qq{16}{4}{1}{50}
\qq{16}{3}{1}{52}
\qq{16}{2}{1}{54}
\qq{16}{1}{1}{56}
\qq{15}{40}{3}{60}
\qq{15}{39}{3}{62}
\qq{15}{38}{3}{64}
\qq{15}{37}{3}{66}
\qq{15}{36}{3}{68}
\qq{15}{35}{3}{70}
\qq{15}{34}{3}{72}
\qq{15}{33}{3}{74}
\qq{15}{32}{3}{76}
\qq{15}{31}{2}{38}
\qq{15}{30}{2}{40}
\qq{15}{29}{2}{42}
\qq{15}{28}{2}{44}
\qq{15}{27}{2}{46}
\qq{15}{26}{2}{48}
\qq{15}{25}{2}{50}
\qq{15}{24}{2}{52}
\qq{15}{23}{2}{54}
\qq{15}{22}{2}{56}
\qq{15}{21}{2}{58}
\qq{15}{20}{2}{60}
\qq{15}{19}{2}{62}
\qq{15}{18}{2}{64}
\qq{15}{17}{2}{66}
\qq{15}{16}{2}{68}
\qq{15}{15}{2}{70}
\qq{15}{14}{2}{72}
\qq{15}{13}{2}{74}
\qq{15}{12}{2}{76}
\qq{15}{11}{2}{78}
\qq{15}{10}{2}{80}
\qq{15}{9}{2}{82}
\qq{15}{8}{1}{44}
\qq{15}{7}{1}{46}
\qq{15}{6}{1}{48}
\qq{15}{5}{1}{50}
\qq{15}{4}{1}{52}
\qq{15}{3}{1}{54}
\qq{15}{2}{1}{56}
\qq{15}{1}{1}{58}
\qq{14}{40}{3}{62}
\qq{14}{39}{3}{64}
\qq{14}{38}{3}{66}
\qq{14}{37}{3}{68}
\qq{14}{36}{3}{70}
\qq{14}{35}{3}{72}
\qq{14}{34}{3}{74}
\qq{14}{33}{3}{76}
\qq{14}{32}{2}{38}
\qq{14}{31}{2}{40}
\qq{14}{30}{2}{42}
\qq{14}{29}{2}{44}
\qq{14}{28}{2}{46}
\qq{14}{27}{2}{48}
\qq{14}{26}{2}{50}
\qq{14}{25}{2}{52}
\qq{14}{24}{2}{54}
\qq{14}{23}{2}{56}
\qq{14}{22}{2}{58}
\qq{14}{21}{2}{60}
\qq{14}{20}{2}{62}
\qq{14}{19}{2}{64}
\qq{14}{18}{2}{66}
\qq{14}{17}{2}{68}
\qq{14}{16}{2}{70}
\qq{14}{15}{2}{72}
\qq{14}{14}{2}{74}
\qq{14}{13}{2}{76}
\qq{14}{12}{2}{78}
\qq{14}{11}{2}{80}
\qq{14}{10}{2}{82}
\qq{14}{9}{2}{84}
\qq{14}{8}{1}{46}
\qq{14}{7}{1}{48}
\qq{14}{6}{1}{50}
\qq{14}{5}{1}{52}
\qq{14}{4}{1}{54}
\qq{14}{3}{1}{56}
\qq{14}{2}{1}{58}
\qq{14}{1}{1}{60}
\qq{13}{40}{3}{64}
\qq{13}{39}{3}{66}
\qq{13}{38}{3}{68}
\qq{13}{37}{3}{70}
\qq{13}{36}{3}{72}
\qq{13}{35}{3}{74}
\qq{13}{34}{3}{76}
\qq{13}{33}{3}{78}
\qq{13}{32}{2}{40}
\qq{13}{31}{2}{42}
\qq{13}{30}{2}{44}
\qq{13}{29}{2}{46}
\qq{13}{28}{2}{48}
\qq{13}{27}{2}{50}
\qq{13}{26}{2}{52}
\qq{13}{25}{2}{54}
\qq{13}{24}{2}{56}
\qq{13}{23}{2}{58}
\qq{13}{22}{2}{60}
\qq{13}{21}{2}{62}
\qq{13}{20}{2}{64}
\qq{13}{19}{2}{66}
\qq{13}{18}{2}{68}
\qq{13}{17}{2}{70}
\qq{13}{16}{2}{72}
\qq{13}{15}{2}{74}
\qq{13}{14}{2}{76}
\qq{13}{13}{2}{78}
\qq{13}{12}{2}{80}
\qq{13}{11}{2}{82}
\qq{13}{10}{2}{84}
\qq{13}{9}{2}{86}
\qq{13}{8}{1}{48}
\qq{13}{7}{1}{50}
\qq{13}{6}{1}{52}
\qq{13}{5}{1}{54}
\qq{13}{4}{1}{56}
\qq{13}{3}{1}{58}
\qq{13}{2}{1}{60}
\qq{13}{1}{1}{62}
\qq{12}{40}{3}{66}
\qq{12}{39}{3}{68}
\qq{12}{38}{3}{70}
\qq{12}{37}{3}{72}
\qq{12}{36}{3}{74}
\qq{12}{35}{3}{76}
\qq{12}{34}{3}{78}
\qq{12}{33}{2}{40}
\qq{12}{32}{2}{42}
\qq{12}{31}{2}{44}
\qq{12}{30}{2}{46}
\qq{12}{29}{2}{48}
\qq{12}{28}{2}{50}
\qq{12}{27}{2}{52}
\qq{12}{26}{2}{54}
\qq{12}{25}{2}{56}
\qq{12}{24}{2}{58}
\qq{12}{23}{2}{60}
\qq{12}{22}{2}{62}
\qq{12}{21}{2}{64}
\qq{12}{20}{2}{66}
\qq{12}{19}{2}{68}
\qq{12}{18}{2}{70}
\qq{12}{17}{2}{72}
\qq{12}{16}{2}{74}
\qq{12}{15}{2}{76}
\qq{12}{14}{2}{78}
\qq{12}{13}{2}{80}
\qq{12}{12}{2}{82}
\qq{12}{11}{2}{84}
\qq{12}{10}{1}{46}
\qq{12}{9}{1}{48}
\qq{12}{8}{1}{50}
\qq{12}{7}{1}{52}
\qq{12}{6}{1}{54}
\qq{12}{5}{1}{56}
\qq{12}{4}{1}{58}
\qq{12}{3}{1}{60}
\qq{12}{2}{1}{62}
\qq{12}{1}{1}{64}
\qq{11}{40}{3}{68}
\qq{11}{39}{3}{70}
\qq{11}{38}{3}{72}
\qq{11}{37}{3}{74}
\qq{11}{36}{3}{76}
\qq{11}{35}{3}{78}
\qq{11}{34}{3}{80}
\qq{11}{33}{2}{42}
\qq{11}{32}{2}{44}
\qq{11}{31}{2}{46}
\qq{11}{30}{2}{48}
\qq{11}{29}{2}{50}
\qq{11}{28}{2}{52}
\qq{11}{27}{2}{54}
\qq{11}{26}{2}{56}
\qq{11}{25}{2}{58}
\qq{11}{24}{2}{60}
\qq{11}{23}{2}{62}
\qq{11}{22}{2}{64}
\qq{11}{21}{2}{66}
\qq{11}{20}{2}{68}
\qq{11}{19}{2}{70}
\qq{11}{18}{2}{72}
\qq{11}{17}{2}{74}
\qq{11}{16}{2}{76}
\qq{11}{15}{2}{78}
\qq{11}{14}{2}{80}
\qq{11}{13}{2}{82}
\qq{11}{12}{2}{84}
\qq{11}{11}{2}{86}
\qq{11}{10}{1}{48}
\qq{11}{9}{1}{50}
\qq{11}{8}{1}{52}
\qq{11}{7}{1}{54}
\qq{11}{6}{1}{56}
\qq{11}{5}{1}{58}
\qq{11}{4}{1}{60}
\qq{11}{3}{1}{62}
\qq{11}{2}{1}{64}
\qq{11}{1}{1}{66}
\qq{10}{40}{3}{70}
\qq{10}{39}{3}{72}
\qq{10}{38}{3}{74}
\qq{10}{37}{3}{76}
\qq{10}{36}{3}{78}
\qq{10}{35}{3}{80}
\qq{10}{34}{2}{42}
\qq{10}{33}{2}{44}
\qq{10}{32}{2}{46}
\qq{10}{31}{2}{48}
\qq{10}{30}{2}{50}
\qq{10}{29}{2}{52}
\qq{10}{28}{2}{54}
\qq{10}{27}{2}{56}
\qq{10}{26}{2}{58}
\qq{10}{25}{2}{60}
\qq{10}{24}{2}{62}
\qq{10}{23}{2}{64}
\qq{10}{22}{2}{66}
\qq{10}{21}{2}{68}
\qq{10}{20}{2}{70}
\qq{10}{19}{2}{72}
\qq{10}{18}{2}{74}
\qq{10}{17}{2}{76}
\qq{10}{16}{2}{78}
\qq{10}{15}{2}{80}
\qq{10}{14}{2}{82}
\qq{10}{13}{2}{84}
\qq{10}{12}{2}{86}
\qq{10}{11}{1}{48}
\qq{10}{10}{1}{50}
\qq{10}{9}{1}{52}
\qq{10}{8}{1}{54}
\qq{10}{7}{1}{56}
\qq{10}{6}{1}{58}
\qq{10}{5}{1}{60}
\qq{10}{4}{1}{62}
\qq{10}{3}{1}{64}
\qq{10}{2}{1}{66}
\qq{10}{1}{1}{68}
\qq{9}{40}{3}{72}
\qq{9}{39}{3}{74}
\qq{9}{38}{3}{76}
\qq{9}{37}{3}{78}
\qq{9}{36}{2}{40}
\qq{9}{35}{2}{42}
\qq{9}{34}{2}{44}
\qq{9}{33}{2}{46}
\qq{9}{32}{2}{48}
\qq{9}{31}{2}{50}
\qq{9}{30}{2}{52}
\qq{9}{29}{2}{54}
\qq{9}{28}{2}{56}
\qq{9}{27}{2}{58}
\qq{9}{26}{2}{60}
\qq{9}{25}{2}{62}
\qq{9}{24}{2}{64}
\qq{9}{23}{2}{66}
\qq{9}{22}{2}{68}
\qq{9}{21}{2}{70}
\qq{9}{20}{2}{72}
\qq{9}{19}{2}{74}
\qq{9}{18}{2}{76}
\qq{9}{17}{2}{78}
\qq{9}{16}{2}{80}
\qq{9}{15}{2}{82}
\qq{9}{14}{2}{84}
\qq{9}{13}{2}{86}
\qq{9}{12}{1}{48}
\qq{9}{11}{1}{50}
\qq{9}{10}{1}{52}
\qq{9}{9}{1}{54}
\qq{9}{8}{1}{56}
\qq{9}{7}{1}{58}
\qq{9}{6}{1}{60}
\qq{9}{5}{1}{62}
\qq{9}{4}{1}{64}
\qq{9}{3}{1}{66}
\qq{9}{2}{1}{68}
\qq{9}{1}{1}{70}
\qq{8}{40}{3}{74}
\qq{8}{39}{3}{76}
\qq{8}{38}{2}{38}
\qq{8}{37}{2}{40}
\qq{8}{36}{2}{42}
\qq{8}{35}{2}{44}
\qq{8}{34}{2}{46}
\qq{8}{33}{2}{48}
\qq{8}{32}{2}{50}
\qq{8}{31}{2}{52}
\qq{8}{30}{2}{54}
\qq{8}{29}{2}{56}
\qq{8}{28}{2}{58}
\qq{8}{27}{2}{60}
\qq{8}{26}{2}{62}
\qq{8}{25}{2}{64}
\qq{8}{24}{2}{66}
\qq{8}{23}{2}{68}
\qq{8}{22}{2}{70}
\qq{8}{21}{2}{72}
\qq{8}{20}{2}{74}
\qq{8}{19}{2}{76}
\qq{8}{18}{2}{78}
\qq{8}{17}{2}{80}
\qq{8}{16}{2}{82}
\qq{8}{15}{1}{44}
\qq{8}{14}{1}{46}
\qq{8}{13}{1}{48}
\qq{8}{12}{1}{50}
\qq{8}{11}{1}{52}
\qq{8}{10}{1}{54}
\qq{8}{9}{1}{56}
\qq{8}{8}{1}{58}
\qq{8}{7}{1}{60}
\qq{8}{6}{1}{62}
\qq{8}{5}{1}{64}
\qq{8}{4}{1}{66}
\qq{8}{3}{1}{68}
\qq{8}{2}{1}{70}
\qq{8}{1}{1}{72}
\qq{7}{40}{2}{36}
\qq{7}{39}{2}{38}
\qq{7}{38}{2}{40}
\qq{7}{37}{2}{42}
\qq{7}{36}{2}{44}
\qq{7}{35}{2}{46}
\qq{7}{34}{2}{48}
\qq{7}{33}{2}{50}
\qq{7}{32}{2}{52}
\qq{7}{31}{2}{54}
\qq{7}{30}{2}{56}
\qq{7}{29}{2}{58}
\qq{7}{28}{2}{60}
\qq{7}{27}{2}{62}
\qq{7}{26}{2}{64}
\qq{7}{25}{2}{66}
\qq{7}{24}{2}{68}
\qq{7}{23}{2}{70}
\qq{7}{22}{2}{72}
\qq{7}{21}{2}{74}
\qq{7}{20}{2}{76}
\qq{7}{19}{2}{78}
\qq{7}{18}{2}{80}
\qq{7}{17}{2}{82}
\qq{7}{16}{2}{84}
\qq{7}{15}{1}{46}
\qq{7}{14}{1}{48}
\qq{7}{13}{1}{50}
\qq{7}{12}{1}{52}
\qq{7}{11}{1}{54}
\qq{7}{10}{1}{56}
\qq{7}{9}{1}{58}
\qq{7}{8}{1}{60}
\qq{7}{7}{1}{62}
\qq{7}{6}{1}{64}
\qq{7}{5}{1}{66}
\qq{7}{4}{1}{68}
\qq{7}{3}{1}{70}
\qq{7}{2}{0}{32}
\qq{7}{1}{0}{34}
\qq{6}{40}{2}{38}
\qq{6}{39}{2}{40}
\qq{6}{38}{2}{42}
\qq{6}{37}{2}{44}
\qq{6}{36}{2}{46}
\qq{6}{35}{2}{48}
\qq{6}{34}{2}{50}
\qq{6}{33}{2}{52}
\qq{6}{32}{2}{54}
\qq{6}{31}{2}{56}
\qq{6}{30}{2}{58}
\qq{6}{29}{2}{60}
\qq{6}{28}{2}{62}
\qq{6}{27}{2}{64}
\qq{6}{26}{2}{66}
\qq{6}{25}{2}{68}
\qq{6}{24}{2}{70}
\qq{6}{23}{2}{72}
\qq{6}{22}{2}{74}
\qq{6}{21}{2}{76}
\qq{6}{20}{1}{38}
\qq{6}{19}{1}{40}
\qq{6}{18}{1}{42}
\qq{6}{17}{1}{44}
\qq{6}{16}{1}{46}
\qq{6}{15}{1}{48}
\qq{6}{14}{1}{50}
\qq{6}{13}{1}{52}
\qq{6}{12}{1}{54}
\qq{6}{11}{1}{56}
\qq{6}{10}{1}{58}
\qq{6}{9}{1}{60}
\qq{6}{8}{1}{62}
\qq{6}{7}{1}{64}
\qq{6}{6}{1}{66}
\qq{6}{5}{1}{68}
\qq{6}{4}{0}{30}
\qq{6}{3}{0}{32}
\qq{6}{2}{0}{34}
\qq{6}{1}{0}{36}
\qq{5}{40}{2}{40}
\qq{5}{39}{2}{42}
\qq{5}{38}{2}{44}
\qq{5}{37}{2}{46}
\qq{5}{36}{2}{48}
\qq{5}{35}{2}{50}
\qq{5}{34}{2}{52}
\qq{5}{33}{2}{54}
\qq{5}{32}{2}{56}
\qq{5}{31}{2}{58}
\qq{5}{30}{2}{60}
\qq{5}{29}{2}{62}
\qq{5}{28}{2}{64}
\qq{5}{27}{2}{66}
\qq{5}{26}{2}{68}
\qq{5}{25}{2}{70}
\qq{5}{24}{2}{72}
\qq{5}{23}{2}{74}
\qq{5}{22}{1}{36}
\qq{5}{21}{1}{38}
\qq{5}{20}{1}{40}
\qq{5}{19}{1}{42}
\qq{5}{18}{1}{44}
\qq{5}{17}{1}{46}
\qq{5}{16}{1}{48}
\qq{5}{15}{1}{50}
\qq{5}{14}{1}{52}
\qq{5}{13}{1}{54}
\qq{5}{12}{1}{56}
\qq{5}{11}{1}{58}
\qq{5}{10}{1}{60}
\qq{5}{9}{1}{62}
\qq{5}{8}{1}{64}
\qq{5}{7}{1}{66}
\qq{5}{6}{0}{28}
\qq{5}{5}{0}{30}
\qq{5}{4}{0}{32}
\qq{5}{3}{0}{34}
\qq{5}{2}{0}{36}
\qq{5}{1}{0}{38}
\qq{4}{40}{2}{42}
\qq{4}{39}{2}{44}
\qq{4}{38}{2}{46}
\qq{4}{37}{2}{48}
\qq{4}{36}{2}{50}
\qq{4}{35}{2}{52}
\qq{4}{34}{2}{54}
\qq{4}{33}{2}{56}
\qq{4}{32}{2}{58}
\qq{4}{31}{2}{60}
\qq{4}{30}{2}{62}
\qq{4}{29}{2}{64}
\qq{4}{28}{2}{66}
\qq{4}{27}{2}{68}
\qq{4}{26}{2}{70}
\qq{4}{25}{2}{72}
\qq{4}{24}{2}{74}
\qq{4}{23}{2}{76}
\qq{4}{22}{1}{38}
\qq{4}{21}{1}{40}
\qq{4}{20}{1}{42}
\qq{4}{19}{1}{44}
\qq{4}{18}{1}{46}
\qq{4}{17}{1}{48}
\qq{4}{16}{1}{50}
\qq{4}{15}{1}{52}
\qq{4}{14}{1}{54}
\qq{4}{13}{1}{56}
\qq{4}{12}{1}{58}
\qq{4}{11}{1}{60}
\qq{4}{10}{1}{62}
\qq{4}{9}{1}{64}
\qq{4}{8}{1}{66}
\qq{4}{7}{1}{68}
\qq{4}{6}{0}{30}
\qq{4}{5}{0}{32}
\qq{4}{4}{0}{34}
\qq{4}{3}{0}{36}
\qq{4}{2}{0}{38}
\qq{4}{1}{0}{40}
\qq{3}{40}{2}{44}
\qq{3}{39}{2}{46}
\qq{3}{38}{2}{48}
\qq{3}{37}{2}{50}
\qq{3}{36}{2}{52}
\qq{3}{35}{2}{54}
\qq{3}{34}{2}{56}
\qq{3}{33}{2}{58}
\qq{3}{32}{2}{60}
\qq{3}{31}{2}{62}
\qq{3}{30}{2}{64}
\qq{3}{29}{2}{66}
\qq{3}{28}{2}{68}
\qq{3}{27}{2}{70}
\qq{3}{26}{2}{72}
\qq{3}{25}{2}{74}
\qq{3}{24}{2}{76}
\qq{3}{23}{1}{38}
\qq{3}{22}{1}{40}
\qq{3}{21}{1}{42}
\qq{3}{20}{1}{44}
\qq{3}{19}{1}{46}
\qq{3}{18}{1}{48}
\qq{3}{17}{1}{50}
\qq{3}{16}{1}{52}
\qq{3}{15}{1}{54}
\qq{3}{14}{1}{56}
\qq{3}{13}{1}{58}
\qq{3}{12}{1}{60}
\qq{3}{11}{1}{62}
\qq{3}{10}{1}{64}
\qq{3}{9}{1}{66}
\qq{3}{8}{1}{68}
\qq{3}{7}{0}{30}
\qq{3}{6}{0}{32}
\qq{3}{5}{0}{34}
\qq{3}{4}{0}{36}
\qq{3}{3}{0}{38}
\qq{3}{2}{0}{40}
\qq{3}{1}{0}{42}
\qq{2}{40}{2}{46}
\qq{2}{39}{2}{48}
\qq{2}{38}{2}{50}
\qq{2}{37}{2}{52}
\qq{2}{36}{2}{54}
\qq{2}{35}{2}{56}
\qq{2}{34}{2}{58}
\qq{2}{33}{2}{60}
\qq{2}{32}{2}{62}
\qq{2}{31}{2}{64}
\qq{2}{30}{2}{66}
\qq{2}{29}{2}{68}
\qq{2}{28}{2}{70}
\qq{2}{27}{2}{72}
\qq{2}{26}{2}{74}
\qq{2}{25}{2}{76}
\qq{2}{24}{2}{78}
\qq{2}{23}{1}{40}
\qq{2}{22}{1}{42}
\qq{2}{21}{1}{44}
\qq{2}{20}{1}{46}
\qq{2}{19}{1}{48}
\qq{2}{18}{1}{50}
\qq{2}{17}{1}{52}
\qq{2}{16}{1}{54}
\qq{2}{15}{1}{56}
\qq{2}{14}{1}{58}
\qq{2}{13}{1}{60}
\qq{2}{12}{1}{62}
\qq{2}{11}{1}{64}
\qq{2}{10}{1}{66}
\qq{2}{9}{1}{68}
\qq{2}{8}{0}{30}
\qq{2}{7}{0}{32}
\qq{2}{6}{0}{34}
\qq{2}{5}{0}{36}
\qq{2}{4}{0}{38}
\qq{2}{3}{0}{40}
\qq{2}{2}{0}{42}
\qq{2}{1}{0}{44}
\qq{1}{40}{2}{48}
\qq{1}{39}{2}{50}
\qq{1}{38}{2}{52}
\qq{1}{37}{2}{54}
\qq{1}{36}{2}{56}
\qq{1}{35}{2}{58}
\qq{1}{34}{2}{60}
\qq{1}{33}{2}{62}
\qq{1}{32}{2}{64}
\qq{1}{31}{2}{66}
\qq{1}{30}{2}{68}
\qq{1}{29}{2}{70}
\qq{1}{28}{2}{72}
\qq{1}{27}{1}{34}
\qq{1}{26}{1}{36}
\qq{1}{25}{1}{38}
\qq{1}{24}{1}{40}
\qq{1}{23}{1}{42}
\qq{1}{22}{1}{44}
\qq{1}{21}{1}{46}
\qq{1}{20}{1}{48}
\qq{1}{19}{1}{50}
\qq{1}{18}{1}{52}
\qq{1}{17}{1}{54}
\qq{1}{16}{1}{56}
\qq{1}{15}{1}{58}
\qq{1}{14}{1}{60}
\qq{1}{13}{1}{62}
\qq{1}{12}{1}{64}
\qq{1}{11}{1}{66}
\qq{1}{10}{1}{68}
\qq{1}{9}{1}{70}
\qq{1}{8}{0}{32}
\qq{1}{7}{0}{34}
\qq{1}{6}{0}{36}
\qq{1}{5}{0}{38}
\qq{1}{4}{0}{40}
\qq{1}{3}{0}{42}
\qq{1}{2}{0}{44}
\qq{1}{1}{0}{46}

